System identification of neural systems: If we got it right, would we know?

Artificial neural networks are being proposed as models of parts of the brain. The networks are compared to recordings of biological neurons, and good performance in reproducing neural responses is considered to support the model's validity. A key question is how much this system identification approach tells us about brain computation. Does it validate one model architecture over another? We evaluate the most commonly used comparison techniques, such as a linear encoding model and centered kernel alignment, to correctly identify a model by replacing brain recordings with known ground truth models. System identification performance is quite variable; it also depends significantly on factors independent of the ground truth architecture, such as stimuli images. In addition, we show the limitations of using functional similarity scores in identifying higher-level architectural motifs.

==> sections/future_work_and_broader_impacts.tex <==
Neural networks have been proven \citep{yamins2014performance} to be able to reproduce neural data. This is good but not too surprising because linear regression on random features can yield  universal approximation \citep{NIPS2008_0efe3284, DBLP:journals/corr/abs-1904-00687}. From the point of view of a neuroscientist, the problem is that several rather different architectures seem to be able to account rather well for the neural data, with differences among them that may be too small or too inconsistent to be of sufficiently clear significance.

At least since the Neocognitron \citep{fukushima:1980} and HMAX \citep{Serre2007}, networks that can readily learn from data have led to models which can better explain neuroscience data. However, the ability to learn from data can potentially become a confound, obscuring well-understood underlying factors that lead to accurate identification of biological systems. It is worthwhile to think about the history of models in neuroscience to appreciate some of the potential risks of these new approaches. Until now most of the biological models were well motivated by various aspects of the underlying neuroscience, usually spanning several different experimental methods such as anatomy, physiology and biophysics. 

Recently, however, researchers begun to use models that were developed by the engineering community without any direct neuroscience constraint and then to evaluate them solely on their ability to reproduce neural activities. An interesting example is offered by \citep{CHANG20212785}, which compares many different models with respect to their ability of reproducing neural responses in IT to face images and conclude that the {\it 2D morphable model} is best. Such a model, originally proposed for faces by \citep{Jones1998MultidimensionalMM}, happens to be  the least biologically plausible among all the models considered, requiring operations such as correspondence and vectorization that do not have an obvious biological implementation in terms of neurons and synapses. 
As we argued earlier, ranking models this way is only the first step in the verification or falsification of a neuroscience model. From this point of view, it is quite possible that architectural validation will have to be done independently of functional validation. It is also quite possible that especially designed stimuli may provide at least initial evidence for different architectures from functional measurements alone. As a simple example, it may be possible to discriminate between dense and local (e.g. CNN) networks by measuring the presence or absence of interactions between parts of a visual stimulus that are spatially separated.  The growing synergies between neuroscience and machine learning clearly require the development of a more comprehensive validation framework of networks models of the brain.
